Boosting Reasoning in Large Multimodal Models via Activation Replay

Recently, Reinforcement Learning with Verifiable Rewards (RLVR) has emerged as an effective approach to incentivizing reasoning capability in Large Multimodal Models (LMMs), while the underlying mechanisms behind this post-training paradigm are poorly understood. We begin by exploring how input activations are affected by RLVR through the perspective of logit lens. Our systematic investigations across multiple post-trained LMMs suggest that RLVR shifts low-entropy activations unexpectedly, while high-entropy ones are less affected. We further demonstrate that such phenomena are associated with LMM reasoning by controlled experiments, suggesting a potentially beneficial role of modulating low-entropy activations. To this end, we propose Activation Replay, a novel simple yet effective training-free approach that boosts multimodal reasoning of post-trained LMMs without requiring expensive policy optimization. Our design involves manipulation of visual tokens at test time, replaying low-entropy activations from the input context of base LMMs to regulating the RLVR counterparts. Activation Replay triggers better reasoning across diverse scenarios, including mathematics, o3-like visual agents, and video reasoning. We further show that Activation Replay boosts Pass@K and mitigates narrower reasoning coverage of RLVR. Our design is compared against alternative choices, such as replaying high-entropy activations instead of low-entropy ones, or direct cross-model intervention instead of manipulating input tokens, demonstrating the superiority of our implementation. Code is publicly available at https://github.com/latentcraft/replay.

==> tab/tf_visionreasoner.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Activation Replay on VisionReasoner~\cite{liu2025visionreasoner}.}
    \label{tab:tf_segzero}
    \begin{small}
    \renewcommand{\arraystretch}{1.0}
        \begin{tabularx}{\linewidth}{p{0.4\linewidth}*{4}{>{\centering\arraybackslash}X}}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & 
        \multicolumn{2}{c}{\textbf{ReasonSeg}} & 
        \multicolumn{2}{c}{\textbf{PixMo}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        & \textit{val} & \textit{test} & \textit{val} & \textit{test} \\
        \midrule
        LLaVA-OV-7B~\cite{li2024llavaov} & -- & -- & 55.8 & 53.7 \\
        Qwen2-VL-7B~\cite{wang2024qwen2vl} & 44.5 & 38.7 & 29.9 & 48.0 \\
        Qwen2.5-VL-7B~\cite{bai2025qwen2_5_vl} & 56.9 & 52.1 & 63.3 & 67.9 \\
        SegZero-7B~\cite{liu2025segzero} & 62.6 & 57.5 & -- & --\\
        \midrule
        VisionReasoner-7B~\cite{liu2025visionreasoner} & \gray{66.3} & \gray{63.6} & \gray{70.1} & \gray{69.5} \\
        & 65.9 & 63.3 & 72.0 & 70.9 \\
        \rowcolor{gray!15}\textit{+ replay} & \textbf{--} & \textbf{--} & \textbf{--} & \textbf{--} \\
        \bottomrule
        \end{tabularx}
    \end{small}
\end{table}
